Revisiting $\Psi$DONet: microlocally inspired filters for incomplete-data tomographic reconstructions

In this paper, we revisit a supervised learning approach based on unrolling, known as $\Psi$DONet, by providing a deeper microlocal interpretation for its theoretical analysis, and extending its study to the case of sparse-angle tomography. Furthermore, we refine the implementation of the original $\Psi$DONet considering special filters whose structure is specifically inspired by the streak artifact singularities characterizing tomographic reconstructions from incomplete data. This allows to considerably lower the number of (learnable) parameters while preserving (or even slightly improving) the same quality for the reconstructions from limited-angle data and providing a proof-of-concept for the case of sparse-angle tomographic data.

==> images/LA30/10564.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/gt_10564.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_square_filter_10564.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uubow{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_bowtie_filter_offset_0_10564.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_x_filter_offset_0_10564.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_x_filter_offset_1_10564.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the reconstructions for the image 10564 with $A=[-\pi/3,\pi/3]$.}
    \label{fig:LA30_10564}
\end{figure}

==> images/LA30/10589.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/gt_10589.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_square_filter_10589.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uubow{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_bowtie_filter_offset_0_10589.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_x_filter_offset_0_10589.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_x_filter_offset_1_10589.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the reconstructions for the image 10589 with $A=[-\pi/3,\pi/3]$.}
    \label{fig:LA30_10589}
\end{figure}

==> images/LA30/10825.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/gt_10825.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_square_filter_10825.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uubow{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_bowtie_filter_offset_0_10825.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_x_filter_offset_0_10825.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA30/LA_x_filter_offset_1_10825.png}};
	\spy on (0.8,0.4) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.5,0.2) in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the reconstructions for the image 10825 with $A=[-\pi/3,\pi/3]$.}
    \label{fig:LA30_10825}
\end{figure}

==> images/LA60/10567.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/gt_10567.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_square_filter_10567.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uubow{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_bowtie_filter_offset_0_10567.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_x_filter_offset_0_10567.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_x_filter_offset_1_10567.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10567 with limited angle in $[-\pi/6,\pi/6]$.}
    \label{fig:LA60_10567}
\end{figure}

==> images/LA60/10825.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/gt_10825.png}};
	\spy on (0.5,-0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.2,0.35)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_square_filter_10825.png}};
	\spy on (0.5,-0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.2,0.35)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uubow{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_bowtie_filter_offset_0_10825.png}};
	\spy on (0.5,-0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.2,0.35)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_x_filter_offset_0_10825.png}};
	\spy on (0.5,-0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.2,0.35)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_x_filter_offset_1_10825.png}};
	\spy on (0.5,-0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.2,0.35)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10825 with limited angle in $[-\pi/6,\pi/6]$.}
    \label{fig:LA60_10825}
\end{figure}

==> images/LA60/10863.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/gt_10863.png}};
	\spy on (0.85,0.35) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_square_filter_10863.png}};
	\spy on (0.85,0.35) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uubow{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_bowtie_filter_offset_0_10863.png}};
	\spy on (0.85,0.35) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{0}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_x_filter_offset_0_10863.png}};
	\spy on (0.85,0.35) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uux{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/LA60/LA60_x_filter_offset_1_10863.png}};
	\spy on (0.85,0.35) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10863 with limited angle in $[-\pi/6,\pi/6]$.}
    \label{fig:LA60_10863}
\end{figure}

==> images/sparse15/10743.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/gt_10743.png}};
	\spy on (0.95,-0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,0.3)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/SPARSE_step_15_square_filter_double_10743.png}};
	\spy on (0.95,-0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,0.3)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uuspa{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/SPARSE_step_15_x_filter_double_offset1_10743.png}};
	\spy on (0.95,-0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,0.3)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10743 for 12 sparse angles.}
    \label{fig:sparse15_10743}
\end{figure}

==> images/sparse15/10919.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/gt_10919.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/SPARSE_step_15_square_filter_double_10919.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uuspa{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/SPARSE_step_15_x_filter_double_offset1_10919.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10919 for 12 sparse angles.}
    \label{fig:sparse15_10919}
\end{figure}

==> images/sparse15/10931.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/gt_10931.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/SPARSE_step_15_square_filter_double_10931.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uuspa{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse15/SPARSE_step_15_x_filter_double_offset1_10931.png}};
	\spy on (0.85,0.65) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10931 for 12 sparse angles.}
    \label{fig:sparse15_10931}
\end{figure}

==> images/sparse30/10521.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/gt_10521.png}};
	\spy on (0.75,0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/SPARSE_30_square_filter_double_10521.png}};
	\spy on (0.75,0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uuspa{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/SPARSE_30_x_filter_double_offset1_10521.png}};
	\spy on (0.75,0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,-0.6)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10521 for 6 sparse angles.}
    \label{fig:sparse30_10521}
\end{figure}

==> images/sparse30/10631.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/gt_10631.png}};
	\spy on (0.70,0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (0.00,-0.5)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/SPARSE_30_square_filter_double_10631.png}};
	\spy on (0.70,0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (0.00,-0.5)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uuspa{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/SPARSE_30_x_filter_double_offset1_10631.png}};
	\spy on (0.70,0.75) in node [name=c1]  at (0.75,-2.25);
	\spy on (0.00,-0.5)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10631 for 6 sparse angles.}
    \label{fig:sparse30_10631}
\end{figure}

==> images/sparse30/10969.tex <==
\begin{figure}
	\centering
	\subfloat[GT]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/gt_10969.png}};
	\spy on (0.95,-0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,0.3)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uupsi$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/SPARSE_30_square_filter_double_10969.png}};
	\spy on (0.95,-0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,0.3)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	\subfloat[$\uuspa{1}$]{
	\scalebox{0.8}{
	\begin{tikzpicture}
	\begin{scope}[spy using outlines={rectangle,blue,magnification=2,size=1.5cm}]
	\node [name=c]{	\includegraphics[height=3cm]{images/sparse30/SPARSE_30_x_filter_double_offset1_10969.png}};
	\spy on (0.95,-0.55) in node [name=c1]  at (0.75,-2.25);
	\spy on (-0.6,0.3)  in node [name=c1]  at (-0.75,-2.25);
	\end{scope}
	\end{tikzpicture}}}
	
    \caption{Visualization of the results for the image 10969 for 6 sparse angles.}
    \label{fig:sparse30_10969}
\end{figure}
